Interpreting Interpretations: Organizing Attribution Methods by Criteria

Motivated by distinct, though related, criteria, a growing number of attribution methods have been developed tointerprete deep learning. While each relies on the interpretability of the concept of "importance" and our ability to visualize patterns, explanations produced by the methods often differ. As a result, input attribution for vision models fail to provide any level of human understanding of model behaviour. In this work we expand the foundationsof human-understandable concepts with which attributionscan be interpreted beyond "importance" and its visualization; we incorporate the logical concepts of necessity andsufficiency, and the concept of proportionality. We definemetrics to represent these concepts as quantitative aspectsof an attribution. This allows us to compare attributionsproduced by different methods and interpret them in novelways: to what extent does this attribution (or this method)represent the necessity or sufficiency of the highlighted inputs, and to what extent is it proportional? We evaluate our measures on a collection of methods explaining convolutional neural networks (CNN) for image classification. We conclude that some attribution methods are more appropriate for interpretation in terms of necessity while others are in terms of sufficiency, while no method is always the most appropriate in terms of both.

==> Makefile <==
OS   := $(shell uname)
ifeq ($(OS), Linux)
  OPEN := evince
else
ifneq ("$(wildcard /Applications/Skim.app)","")
  OPEN := open -a /Applications/Skim.app
else
  OPEN := open -a /Applications/Preview.app
endif
endif
DOC  := doc-explanation-evaluation
MAIN := egpaper_for_review
PDFLATEX := pdflatex

DEP_FIGS := $(shell find ./figures \
	-name '*.tex' \
	)
DEP := *.tex *.bib $(DEP_FIGS)
DEP := $(foreach i,$(DEP),$(shell ls $(i) 2> /dev/null))

start:
	make draft

start-%:
	make open-$*
	make watch-$*

draft:
	make start-draft

final:
	make start-final

$(DOC).final.main.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 1-9 output $@

$(DOC).final.supplemental.pdf: $(DOC).final.pdf
	pdftk $(DOC).final.pdf cat 10-12 output $@

parts: $(DOC).final.main.pdf $(DOC).final.supplemental.pdf

startt:
	$(PDFLATEX) $(QUIET) preamble; $(BIBTEX) $(QUIET) $(MAIN); $(PDFLATEX) $(QUIET) preamble; $(PDFLATEX) $(QUIET) preamble;
	make clean; $(OPEN) preamble.pdf

open-%: $(DOC).%.pdf
ifneq ("$(OPEN)","")
	$(OPEN) $(DOC).$*.pdf ; sleep 1
else
	@echo "Could not find a PDF reader. If you'd like this \
	makefile to open the generated pdfs, add your PDF reader to \
	the opening section of the Makefile."
	@exit 1
endif

$(DOC).pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\input{$(MAIN).tex}"
	@cp $(MAIN).pdf $(DOC).pdf
	@cp $(MAIN).synctex.gz $(DOC).synctex.gz


$(DOC).%.pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\def\$*{}\input{$(MAIN).tex}"
	@cp $(MAIN).pdf $(DOC).$*.pdf
	@cp $(MAIN).synctex.gz $(DOC).$*.synctex.gz

watch-%:
	perl watch.pl watch $(DOC).$*.pdf $(DEP)
	perl watch.pl watch $(DOC).pdf $(DEP)

# DEBUGGING UTILS
# https://www.cmcrossroads.com/article/printing-value-makefile-variable
print-%  : ; @echo $* = $($*)

debug: $(DEP)
	$(PDFLATEX) -interaction nonstopmode "\input{$(MAIN).tex}"
	$(OPEN) $(DOC).pdf

# To debug unicode issues:
# useful emacs command: find-file-literally
show_unicode: $(DEP)
	pcregrep --color='auto' -n "[\x80-\xFF]" *.tex *.bib

# List all references to the thing after find_ in the tex sources.
find_%: *.tex
	grep -I -C 1 -n --color=auto '$*' *.tex; true

# CLEANING
clean:
	rm -Rf *.aux *.lof *.log *.lot *.bbl *.blg *.toc *.out *.bcf *.run.xml; true
	rm -Rf *~; true
	rm -Rf $(DOC).pdf $(MAIN).pdf $(DOC).*.pdf; true
	rm -Rf main-blx.bib
	rm -Rf .DS_Store; true
	rm -Rf .iTeXMac; true
	rm -Rf *.*.gz; true
	rm -Rf *.pdfsync; true
	rm -Rf *.synctex; true

desvn:
	find . -type d -name .svn -exec rm -rf {} +

#ARTIFACTS := $(shell find artifact)

#artifact: ${ARTIFACTS}
#	COPYFILE_DISABLE=1 tar -cvf artifact.tar artifact
#	gzip artifact.tar

# PACKAGING

DEP_TEX := $(shell find . \
	-not \( -path ./old-sections -prune \) \
	-not \( -path ./supplemental -prune \) \
	-not \( -path ./ijcai2018-formatting-guidelines -prune \) \
	-not \( -path ./arXiv -prune \) \
	-not \( -path ./formatting_instructions -prune \) \
	-not \( -path ./styles -prune \) \
	-name '*.tex' \
	)

DEP_TEX2 := $(DEP_TEX:%=arXiv/%)

arXiv/%.tex: %.tex
	latexpand --empty-comments $< > arXiv/$<
	sed -e '/^\s*%/d' -i '' arXiv/$<

arXiv:
	mkdir arXiv
	mkdir arXiv/figures

$(MAIN).bbl: $(DOC).arXiv.pdf

bundle: $(MAIN).bbl arXiv $(DEP_TEX:%=arXiv/%) ijcai18.sty
	cp -R $(MAIN).bbl ijcai18.sty arXiv
	cp -R $(DEP_FIGS) arXiv/figures
	(echo "\def\\\\arXiv{}\n"; cat arXiv/$(MAIN).tex) \
           > arXiv/$(MAIN).tex.temp
	mv arXiv/$(MAIN).tex.temp arXiv/$(MAIN).tex
	tar -cvf arXiv.tar arXiv
	gzip arXiv.tar

rebundle:
	rm -Rf arXiv; true
	rm -Rf arXiv.tar.gz; true
	make bundle

